DeepSound-V1: Start to Think Step-by-Step in the Audio Generation from Videos

Currently, high-quality, synchronized audio is synthesized from video and optional text inputs using various multi-modal joint learning frameworks. However, the precise alignment between the visual and generated audio domains remains far from satisfactory. One key factor is the lack of sufficient temporal and semantic alignment annotations in open-source video-audio and text-audio benchmarks. Therefore, we propose a framework for audio generation from videos, leveraging the internal chain-of-thought (CoT) of a multi-modal large language model (MLLM) to enable step-by-step reasoning without requiring additional annotations. Additionally, a corresponding multi-modal reasoning dataset is constructed to facilitate the learning of initial reasoning in audio generation. In the experiments, we demonstrate the effectiveness of the proposed framework in reducing misalignment (voice-over) in generated audio and achieving competitive performance compared to various state-of-the-art models. The evaluation results show that the proposed method outperforms state-of-the-art approaches across multiple metrics. Specifically, the F DP aSST indicator is reduced by up to 10.07%, the F DP AN N s indicator by up to 11.62%, and the F DV GG indicator by up to 38.61%. Furthermore, the IS indicator improves by up to 4.95%, the IB-score indicator increases by up to 6.39%, and the DeSync indicator is reduced by up to 0.89%.

==> tab/large.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]

\centering
\resizebox{\linewidth}{!}{


\begin{tabular}{lcccccccc}
\hline
                                                   & \multicolumn{5}{c}{Distribution matching}                                                                                                                        & Audio quality                & Semantic align                  & Temporal align                \\ \cline{2-9} 

& FD_{PaSST}$\downarrow$ & FD_{PANNs}$\downarrow$ &  FD_{VGG}$\downarrow$ & KL_{PANNs}$\downarrow$ &  KL_{PaSST}$\downarrow$ &  IS$\uparrow$ &  IB-score$\uparrow$ &  DeSync$\downarrow$ \\ \hline
 setting1 \& vggtest-gt1      & 60.60 & 4.72 & 0.97 & 1.65 & 1.40 & 17.40 & 33.22 & 0.442 \\
 setting1 \& vggtest-gt2    &  56.29  &  4.29 &  1.03  &  2.13  &  1.72  &  14.54 &   32.74  &  0.475                            \\
setting1-neg \& vggtest-gt1  &   59.50 &  4.62  &   1.75 & 2.19  & 1.76  &  15.42 & 32.36 &  0.490                             \\ \midrule

% setting2-cot \& vggtest-gt2 &  \textbf{55.65}(\textcolor[HTML]{006400}{10.07\%})   &  4.80   & \textbf{0.93} (\textcolor[HTML]{006400}{17.70\%}) & 2.15   & 1.77   &  13.82 &  31.44    &  0.495  \\
setting2-cot \& vggtest-gt2 & 55.19 & 4.42 & 0.95 & 2.13 & 1.75 & 14.49 & 31.94 & 0.490 \\

setting3-rm \& vggtest-gt2  &  55.75 & 4.49 & 1.00 & 2.12 & 1.73 & 14.70 & 32.25 & 0.484 \\
setting3-rep \& vggtest-gt2 &  55.66 & 4.45 & 0.97 & 2.14 & 1.74 & 14.61 & 32.16 & 0.486 \\
setting3-neg \& vggtest-gt2 &  55.66 & 4.44 & 0.99 & 2.13 & 1.74 & 14.65 & 32.17 & 0.487  \\ \hline
\end{tabular}

}
\caption{Ablation result on MMAudio-large-44k}
\label{table:mmaduio-large-44k}
\end{table*}

==> tab/table3.tex <==
\begin{table}[]
\begin{tabular}{llllll}
method        & human voice ratio from QA detect & human voice ratio from CoT detect & voice-over detect number from QA & voice=over detect number from CoT & total voice-over \\
MMAudio-S-16k & 43.76\%                          & 60.32\%                           & 1651                             & 2183                              & 2262             \\
MMAudio-S-44k & 40.46\%                          & 58.30\%                           & 1072                             & 1455                              & 1525             \\
MMuaido-M-44k & 40.61\%                          & 57.22\%                           & 1322                             & 1726                              & 1820             \\
MMAudio-L-44k & 40.78\%                          & 55.62\%                           & 1304                             & 1675                              & 1772             \\
YingSound     & 39.74\%                          & 55.85\%                           & 1459                             & 1960                              & 2020             \\
FoleyCrafter  & 37.57\%                          & 52.98\%                           & 1220                             & 1647                              & 1708            
\end{tabular}
\label{table:table3}
\end{table}
